Universal Activation Verbalizer: A Unified Framework for Cross-Model Activation Explanation

Activation verbalization explains hidden representations in natural language, but existing methods are mostly limited to self-explanation, where each model explains only its own activations. We introduce Universal Activation Verbalizer (UAV), a framework that uses a shared decoder to explain activations from heterogeneous donor models. UAV learns a lightweight adapter that converts donor activations into soft tokens in decoder's embedding space, and further supports adapter-only transfer by reusing a frozen decoder-side LoRA while training only a new adapter for another donor. Across classification, fact retrieval, and gist summarization, UAV remains competitive with strong self-explanation baselines while enabling cross-model verbalization across model families and scales. Ablations show that decoder-side tuning mainly improves task behavior, whereas the adapter provides the activation-grounded factual and semantic information needed for faithful explanations. Code and data are available at https://github.com/hy-zhao23/ActExp.

==> aux/long-table.tex <==
\begin{small}
% \begin{longtable}
\begin{table}[!h]
    \caption{Inverted examples with varying token lengths}
    \label{tab:token-examples}\vskip-12pt
\end{table}
\scalebox{0.94}{\begin{supertabular}{m{0.8cm}|m{4.1cm}|m{4.1cm}|ccccccc}\toprule
% \caption{Examples of inverted sequence with varying token lengths and recovery rate}\label{tab:tokens}
{Tokens (\#)} & {Ground-truth Sequence} & {Inverted Sequence} & {R1} & {R2} & {RL} & {BS} & {SS} & {ES} & TS \\ \midrule
{\multirow{5}{*}{8}} & {in the Centre-Val de Loire} & {in the Centre-Val de Loire} & {1} & {1} & {1} & {1} & {1} & {1} & 1 \\\cmidrule{2-10}
{} & is   the second era of the Hade & is the third era of the Hade & 0.86 & 0.67 & 0.86 & 0.99 & 1 & 0.8 & 1 \\\cmidrule{2-10}
{} & who enforce New Zealand's regulatory   building control & the enforcement of New Zealand   statutory building control & 0.63 & 0.29 & 0.63 & 0.77 & 0.4 & 0.6 & 1 \\\cmidrule{2-10}
{} & Tyler, the Creator production   discography\textbackslash{}n\textbackslash{}n & Metro Boomin production discography\textbackslash{}n\textbackslash{}n & 0.44 & 0.29 & 0.44 & 0.77 & 0.8 & 1 & 1 \\\cmidrule{2-10}
{} & biologist \textbackslash{}n Stanley Fields (actor) ( & :\textbackslash{}n\textbackslash{}n John Allen (actor) (born & 0.25 & 0 & 0.25 & 0.78 & 0.6 & 0.8 & 0.8 \\ \midrule
\multirow{5}{*}{16} & species within the genus Conus, these snails are predatory and   venomous. & species within the genus Conus,   these snails are predatory and venomous. & 1 & 1 & 1 & 1 & 1 & 1 & 1 \\\cmidrule{2-10}
 & List of shipwrecks in September   1842\textbackslash{}n\textbackslash{}nThe list of ship & List of shipwrecks in January 1840\textbackslash{}n\textbackslash{}nThe list of ship & 0.8 & 0.67 & 0.8 & 0.99 & 0.8 & 0.8 & 1 \\\cmidrule{2-10}
 & 2017 NCAA Division I Softball   Tournament\textbackslash{}n\textbackslash{}nThe 2017 NCAA Division I & 2018 NCAA Division I Women's Soccer Tournament\textbackslash{}n\textbackslash{}nThe 2018 NCAA Division & 0.61 & 0.38 & 0.61 & 0.88 & 0.8 & 0.6 & 0.8 \\\cmidrule{2-10}
 & Rob James\textbackslash{}n\textbackslash{}nRob James may refer   to:\textbackslash{}n\textbackslash{}nRob James (singer) ( & Mark Jones\textbackslash{}n\textbackslash{}nMark Jones may refer to:\textbackslash{}n\textbackslash{}nMark Jones (singer) ( & 0.4 & 0.22 & 0.4 & 0.96 & 0.8 & 1 & 1 \\\cmidrule{2-10}
 & Qi   Yuwu, Julian Hee, Jeanette Aw, Felicia Chin, & , Pierre Png, Chen Hanwei, Felicia Chin, Fann Wong & 0.25 & 0.14 & 0.25 & 0.82 & 0.8 & 1 & 1 \\\midrule
\multirow{6}{*}{32} & 1825 in Wales\textbackslash{}n\textbackslash{}nThis article is about the particular significance of the   year 1825 to Wales and its people.\textbackslash{}n\textbackslash{}nIncumbents\textbackslash{}nPrince of Wales \textbackslash{}u2013 & 1840 in Wales\textbackslash{}n\textbackslash{}nThis article is about the particular significance of the   year 1840 to Wales and its people.\textbackslash{}n\textbackslash{}nIncumbents\textbackslash{}nPrince of Wales \textbackslash{}u2013 & 0.91 & 0.86 & 0.91 & 0.99 & 0.8 & 0.8 & 1 \\\cmidrule{2-10}
 % & the United States Census Bureau, the town   has a total area of 37.7\textbackslash{}u00a0square miles (97.6\textbackslash{}u00a0km\textbackslash{}u00b2), of   which, & the United States Census Bureau,   the town has a total area of 35.1\textbackslash{}u00a0square miles (90.9\textbackslash{}u00a0km\textbackslash{}u00b2), of   which, & 0.81 & 0.7 & 0.81 & 0.99 & 0.8 & 1 & 1 \\\cmidrule{2-10}
 & List of European Championships records in   swimming\textbackslash{}n\textbackslash{}nThe European Championships records in swimming are the fastest   times ever swum in European Swimming Championships' events.\textbackslash{}n\textbackslash{}nLong course   (50 & List of European records in swimming\textbackslash{}n\textbackslash{}nThe following are the current   European records in swimming, as recognized by LEN.\textbackslash{}n\textbackslash{}nLong course (50 m   pool)\textbackslash{}n\textbackslash{}nShort course ( & 0.6 & 0.39 & 0.53 & 0.75 & 0.6 & 0.8 & 1 \\\cmidrule{2-10}
 & Institute of Higher National Defence   Studies.\textbackslash{}n\textbackslash{}nThen, he went to the USA for a Master in International Business   Management at the University of Florida. He began his career in & .\textbackslash{}n\textbackslash{}nHe then studied at the Institut d'\textbackslash{}u00e9tudes politiques de Paris   and at the \textbackslash{}u00c9cole nationale d'administration (ENA). He started his career   in & 0.42 & 0.12 & 0.3 & 0.71 & 0.2 & 0.6 & 0.8 \\\cmidrule{2-10}
 & William Robertson Nicoll\textbackslash{}n\textbackslash{}nSir William   Robertson Nicoll CH LLD (10 October 1851 \textbackslash{}u2013 4 May 1923) was a Scottish   Free Church & John Duncan (minister)\textbackslash{}n\textbackslash{}nJohn Duncan (1 May 1845 \textbackslash{}u2013 6 March 1914),   also known as J. Duncan, was a Free & 0.21 & 0.05 & 0.21 & 0.74 & 0.8 & 0.8 & 0.8 \\\cmidrule{2-10}
 & Alessandro Guiccioli\textbackslash{}n\textbackslash{}nAlessandro   Guiccioli (March 5, 1843 \textbackslash{}u2013 October 3, 1922) & Gustave de Beaumont\textbackslash{}n\textbackslash{}nGustave de Beaumont (March 1, 1840 \textbackslash{}u2013 March 2,   1921) was & 0.09 & 0 & 0.09 & 0.83 & 0.6 & 0.4 & 0.8 \\\midrule
\end{supertabular}}

\newpage

\scalebox{0.94}{\begin{supertabular}{m{0.8cm}|m{4.1cm}|m{4.1cm}|ccccccc}
\toprule
\multirow{5}{*}{64} & Rush Hour 2\textbackslash{}n\textbackslash{}nRush Hour 2 is a 2001 American action comedy film directed   by Brett Ratner and written by Jeff Nathanson, based on the characters   created by Ross LaManna. A sequel to Rush Hour, it is the second installment   in the Rush Hour series and stars Jackie Chan, & Rush Hour 2\textbackslash{}n\textbackslash{}nRush Hour 2 is a 2001 American buddy cop action comedy   film directed by Brett Ratner and written by Jeff Nathanson. It is the sequel   to the 1998 film Rush Hour and the second installment in the Rush Hour film   series. The film stars Jackie Chan, & 0.84 & 0.67 & 0.78 & 0.91 & 0.8 & 1 & 1 \\\cmidrule{2-10}
 & hull length of, a beam of, a height of, and   a draught of. The submarine was powered by two Germaniawerft F46 four-stroke,   six-cylinder supercharged diesel engines producing a total of  for use while surfaced, two AEG GU   460/8\textbackslash{}u201327 double- & . The U-boat had a displacement of    when at the surface and  while   submerged. The U-boat had a total length of, a pressure hull length of, a   beam of, a height of, and a draught of. The submarine was powered by two   Germaniawerft F46 six- & 0.61 & 0.48 & 0.49 & 0.8 & 0.4 & 1 & 1 \\\cmidrule{2-10}
 & the same rights of audience as members of   the Bar of Northern Ireland.\textbackslash{}n\textbackslash{}nThe Advocate General was created as a   separate office upon the devolution of policing and justice powers to the   Northern Ireland Assembly on 12 April 2010.\textbackslash{}n\textbackslash{}nUnlike the Advocate General   for Scotland, the position is not supported by a distinct government   department. & the Scottish Parliament. The   office was created in 1999, and is the equivalent of the Parliamentary   Under-Secretary of State in the United Kingdom Government.\textbackslash{}n\textbackslash{}nThe office is   not a ministerial post, and the holder is not a member of the Scottish   Government. Responsibility for the office is held by the Scottish Secretary. & 0.41 & 0.08 & 0.24 & 0.66 & 0.4 & 0.4 & 0.8 \\\cmidrule{2-10}
 & producer Thom Wilson and released in 1982 as   catalog number VIRUS 10. Singer Jack Grisham credited himself as Jack Ladoga   on the sleeve, following a tradition of using a different pseudonym on each   release both to confuse audiences and to hide his true identity from the   police. Drummer Todd Barnes credited himself & the band's first album, and the   first to feature the band's new lineup. The band members used pseudonyms on   the album, with the exception of guitarist and vocalist John   \textbackslash{}"Baz\textbackslash{}" Bascaran, who used his real name because he was the only   member of the band with a driver's license. Drum & 0.21 & 0.04 & 0.15 & 0.59 & 0.8 & 0.6 & 0.8 \\
 \cmidrule{2-10}
 & Linux kernel.\textbackslash{}n\textbackslash{}nXC3018\textbackslash{}nIt is a variant   that only supports analog reception and DVB-T digital reception.\textbackslash{}n\textbackslash{}nTechnical   specification\textbackslash{}nOutline Dimensions: 7 x 7 x 0.85\textbackslash{}u00a0mm\textbackslash{}nSupply Voltage (DC):   1.8V, 3.3V\textbackslash{}nSystem setting time: & 2010.\textbackslash{}n\textbackslash{}nSpecifications\textbackslash{}nFrequency:   2.4\textbackslash{}u00a0GHz\textbackslash{}nData rate: 1, 2, 5.5, 11\textbackslash{}u00a0Mbps\textbackslash{}nModulation: DSSS\textbackslash{}nPower   consumption: 0.1\textbackslash{}u00a0W\textbackslash{}nOperating temperature: 0\textbackslash{}u00a0\textbackslash{}u00b0C to  70\textbackslash{}u00a0\textbackslash{}u00b0C\textbackslash{}n & 0.09 & 0 & 0.09 & 0.62 & 0 & 0 & 0.8 \\\midrule
\end{supertabular}}
% \end{longtable}
\end{small}

==> aux/prompt.tex <==
\section{Instruction Examples}\label{app:prompt}
We include prompts for GPT-4.1-mini as below.

\subsection{Scoring Instructions}\label{app:struct}
\begin{tcolorbox}[
    enhanced,
    breakable,
    colback=orange!10!white, colframe=blue!5!black,
    arc=2mm,
    boxrule=1pt,
    title={\bfseries Structure Score},
    coltitle=white,
    attach boxed title to top left={yshift=-2mm, xshift=3mm},
    boxed title style={enhanced, colback=blue!5!black, colframe=blue!5!black, arc=2mm, boxrule=0pt},
    top=0.5mm, left=1mm, right=1mm, bottom=0.5mm,
]
\setlength{\parskip}{4pt}
\small
\vskip8pt
\textbf{You are given two sentences:}
\begin{itemize}[nosep, topsep=2pt, itemsep=0pt, parsep=0pt,leftmargin=1.2cm]
    \item[\textbf{[GT]:}] \texttt{self.gt\_sen}
    \item[\textbf{[GEN]:}] \texttt{self.gen\_sen}
\end{itemize}
Evaluate \textbf{Structural Frame Similarity}. Focus on whether [GEN] preserves the core grammatical structure and sentence skeleton of [GT]: same basic clause structure, same number/type of major phrases, similar syntactic relationships, consistent verb tense/aspect.

% \begin{tcolorbox}[enhanced, colback=gray!5, colframe=blue!5!black, arc=2mm, boxrule=1pt, left=1mm, right=1mm, top=2mm, bottom=2mm]
\textbf{Scoring:}
\begin{itemize}[nosep, topsep=2pt, itemsep=0pt, parsep=0pt, style=nextline, leftmargin=0.7cm]
    \item[\textbf{5}:] Identical structure — same words in same order
    \item[\textbf{4}:] Nearly identical — same pattern with entity substitutions or minor reordering
    \item[\textbf{3}:] Moderately similar — core structure maintained but notable changes (e.g., active to passive)
    \item[\textbf{2}:] Somewhat similar — recognizable elements but significant differences
    \item[\textbf{1}:] Minimally similar — only basic sentence type matches
    \item[\textbf{0}:] Completely different structures
\end{itemize}
% \end{tcolorbox}

\textbf{Answer:} \texttt{[ANS] structure: [score]/5}
\end{tcolorbox}

\begin{tcolorbox}[
    enhanced,
    breakable,
    colback=orange!10!white, colframe=blue!5!black,
    arc=2mm,
    boxrule=1pt,
    title={\bfseries Entity Score (Clinical)},
    coltitle=white,
    attach boxed title to top left={yshift=-2mm, xshift=3mm},
    boxed title style={enhanced, colback=blue!5!black, colframe=blue!5!black, arc=2mm, boxrule=0pt},
    top=0.5mm, left=1mm, right=1mm, bottom=0.5mm,
]
\setlength{\parskip}{4pt}
\small\vskip8pt
\textbf{You are given two sentences:}
\begin{itemize}[nosep, topsep=2pt, itemsep=0pt, parsep=0pt, leftmargin=1.2cm]
    \item[\textbf{[GT]:}] \texttt{self.gt\_sen}
    \item[\textbf{[GEN]:}] \texttt{self.gen\_sen}
\end{itemize}
Evaluate the \textbf{Entity/Role Consistency and Plausibility} between these snippets.

\textbf{Clinical Entity Type Matching Rules:}
\begin{itemize}[nosep, topsep=2pt, itemsep=0pt, parsep=0pt, style=nextline, leftmargin=0.7cm]
    \item[-] {Patient Demographics}: Age (±5 years = high), same biological sex
    \item[-] {Symptoms / Chief Complaint}: Same symptom category; penalise crossing body systems
    \item[-] {Diagnosis / Condition}: Same condition class; similar severity
    \item[-] {Medications}: Same drug class or mechanism
    \item[-] {Vital Signs / Lab Values}: Numerical proximity (BP $\pm$10 mmHg, O2 sat $\pm$3\%, glucose $\pm$30 mg/dL)
    \item[-] {Anatomical Location}: Same body region or system
    \item[-] {Dates / Admission Timing}: ±30 days = high, ±1 year = moderate, >5 years = low
    \item[-] {Medical Procedures}: Same procedure category
\end{itemize}

\textbf{Scoring Guidelines:} 0–5

\textbf{Answer}: \texttt{[ANS] entity: [score]/5}
\end{tcolorbox}

\begin{tcolorbox}[
    enhanced,
    breakable,
    colback=orange!10!white, colframe=blue!5!black,
    arc=2mm,
    boxrule=1pt,
    title={\bfseries Entity Score (Wiki)},
    coltitle=white,
    attach boxed title to top left={yshift=-2mm, xshift=3mm},
    boxed title style={enhanced, colback=blue!5!black, colframe=blue!5!black, arc=2mm, boxrule=0pt},
    top=0.5mm, left=1mm, right=1mm, bottom=0.5mm,
]
\setlength{\parskip}{4pt}
\small\vskip8pt
\textbf{You are given two sentences:}
\begin{itemize}[nosep, topsep=2pt, itemsep=0pt, parsep=0pt, leftmargin=1.2cm]
    \item[\textbf{[GT]:}] \texttt{self.gt\_sen}
    \item[\textbf{[GEN]:}] \texttt{self.gen\_sen}
\end{itemize}
Evaluate \textbf{Entity Preservation}. Focus on whether [GEN] preserves key entities (people, places, organizations) from [GT]: same named entities, same key objects/concepts, equivalent entities in corresponding roles, preservation of entity relationships.

\textbf{Scoring:}
\begin{itemize}[nosep, topsep=2pt, itemsep=0pt, parsep=0pt, style=nextline, leftmargin=0.7cm]
    \item[\textbf{5}:] All entities preserved — all key entities from GT appear in GEN with same references
    \item[\textbf{4}:] Nearly all preserved — minor omissions of non-critical entities or slight variations
    \item[\textbf{3}:] Most preserved — majority of key entities maintained, some important ones missing/substituted
    \item[\textbf{2}:] Some preserved — recognizable overlap but significant differences in key entities
    \item[\textbf{1}:] Few preserved — minimal overlap, only generic categories match
    \item[\textbf{0}:] No overlap — completely different entities
\end{itemize}

\textbf{Answer:} \texttt{[ANS] entity: [score]/5}
\end{tcolorbox}

\begin{tcolorbox}[
    enhanced,
    breakable,
    colback=orange!10!white, colframe=blue!5!black,
    arc=2mm,
    boxrule=1pt,
    title={\bfseries Topic Score (Wiki)},
    coltitle=white,
    attach boxed title to top left={yshift=-2mm, xshift=3mm},
    boxed title style={enhanced, colback=blue!5!black, colframe=blue!5!black, arc=2mm, boxrule=0pt},
    top=0.5mm, left=1mm, right=1mm, bottom=0.5mm,
]
\setlength{\parskip}{4pt}
\small\vskip8pt
\textbf{You are given two sentences:}
\begin{itemize}[nosep, topsep=2pt, itemsep=0pt, parsep=0pt, leftmargin=1.2cm]
    \item[\textbf{[GT]:}] \texttt{self.gt\_sen}
    \item[\textbf{[GEN]:}] \texttt{self.gen\_sen}
\end{itemize}
Evaluate \textbf{Topic Consistency}. Focus on whether [GEN] maintains the same main subject/topic as [GT]: same primary entity/concept, same domain/field, same general subject matter, maintains relevance to original topic.

\textbf{Scoring:}
\begin{itemize}[nosep, topsep=2pt, itemsep=0pt, parsep=0pt, style=nextline, leftmargin=0.7cm]
    \item[\textbf{5}:] Identical topic — exactly the same specific topic/entity with same focus
    \item[\textbf{4}:] Highly similar — same main topic with slightly different aspects/perspectives
    \item[\textbf{3}:] Related topic — closely related subjects within same domain/category
    \item[\textbf{2}:] Loosely related — some connection but notably different topics/focuses
    \item[\textbf{1}:] Minimally related — tangentially connected or only shares broad category
    \item[\textbf{0}:] Unrelated — completely different subjects with no meaningful connection
\end{itemize}

\textbf{Answer:} \texttt{[ANS] topic: [score]/5}
\end{tcolorbox}

\begin{tcolorbox}[
    enhanced,
    breakable,
    colback=orange!10!white, colframe=blue!5!black,
    arc=2mm,
    boxrule=1pt,
    title={\bfseries Topic Score (Clinical)},
    coltitle=white,
    attach boxed title to top left={yshift=-2mm, xshift=3mm},
    boxed title style={enhanced, colback=blue!5!black, colframe=blue!5!black, arc=2mm, boxrule=0pt},
    top=0.5mm, left=1mm, right=1mm, bottom=0.5mm,
]
\setlength{\parskip}{4pt}
\small\vskip8pt
\textbf{You are given two clinical text snippets:}
\begin{itemize}[nosep, topsep=2pt, itemsep=0pt, parsep=0pt, leftmargin=1.2cm]
    \item[\textbf{[GT]:}] \texttt{self.gt\_sen}
    \item[\textbf{[GEN]:}] \texttt{self.gen\_sen}
\end{itemize}

Evaluate the \textbf{Topical Relevance} between these snippets.

\textbf{Clinical Topic Categories}:
    Cardiology / Pulmonology / Infectious Disease / Neurology / Gastroenterology /
    Endocrinology / Musculoskeletal / Mental Health / Nephrology / General \& Post-op


\textbf{Scoring Guidelines:} 0-5
\begin{itemize}[nosep, topsep=2pt, itemsep=0pt, parsep=0pt, style=nextline, leftmargin=0.7cm]
    \item[\textbf{5}:] Same specific clinical topic (same disease/condition/care scenario)
    \item[\textbf{4}:] Same clinical domain with minor shifts
    \item[\textbf{3}:] Related clinical domains
    \item[\textbf{2}:] Loosely related
    \item[\textbf{1}:] Both clinical but completely different physiological systems
    \item[\textbf{0}:] No meaningful clinical connection
\end{itemize}

\textbf{Answer}: \texttt{[ANS] topic: [score]/5}
\end{tcolorbox}

\subsection{System Prompt}\label{app:sys-prop}

\begin{tcolorbox}[
    enhanced,
    breakable,
    colback=orange!10!white, colframe=blue!5!black,
    arc=2mm,
    boxrule=1pt,
    title={\bfseries System Prompt},
    coltitle=white,
    attach boxed title to top left={yshift=-2mm, xshift=3mm},
    boxed title style={enhanced, colback=blue!5!black, colframe=blue!5!black, arc=2mm, boxrule=0pt},
    top=0.5mm, left=1mm, right=1mm, bottom=0.5mm,
]
% \setlength{\parskip}{4pt}
\small\vskip8pt
You are an AI assistant that can decode the hidden representation vector from the intermediate layer of a language model. You receive a hidden representation vector, which is the representation of an input textual sequence's final token at a fixed layer. The ask is using this representation vector to completely reveal the original text it encodes. Always produce the possible input text as exactly as you can, and avoid rephrasing it.

\end{tcolorbox}


\subsection{User Prompt Examples}\label{app:sys-prop}

\begin{tcolorbox}[
    enhanced,
    breakable,
    colback=orange!10!white, colframe=blue!5!black,
    arc=2mm,
    boxrule=1pt,
    title={\bfseries User Prompts},
    coltitle=white,
    attach boxed title to top left={yshift=-2mm, xshift=3mm},
    boxed title style={enhanced, colback=blue!5!black, colframe=blue!5!black, arc=2mm, boxrule=0pt},
    top=0.5mm, left=1mm, right=1mm, bottom=0.5mm,
]
\setlength{\parskip}{4pt}
\small\vskip8pt

\begin{itemize}
    \item What type of context is this representation most likely encoding?
    \item What does this embedding reveal about the input sequence?
    \item Describe the underlying meaning this hidden state is capturing. 
    \item What kind of sentence or phrase could generate this vector?
    \item What semantic information is likely contained in this hidden representation?
    \item What real-world context could this representation be associated with?
    \item What kind of textual environment might lead to this hidden state?
    \item What is the most plausible meaning encoded by this internal representation?
\end{itemize}
\end{tcolorbox}
\clearpage
